Higher-Order Bayesian Networks, Exactly (Extended version)

Bayesian networks (BNs) are graphical \emph{first-order} probabilistic models that allow for a compact representation of large probability distributions, and for efficient inference, both exact and approximate. We introduce a \emph{higher-order} programming language -- in the idealized form of a $\lambda$-calculus -- which we prove \emph{sound and complete} w.r.t. BNs: each BN can be encoded as a term, and conversely each (possibly higher-order and recursive) program of ground type \emph{compiles} into a BN. The language allows for the specification of recursive probability models and hierarchical structures. Moreover, we provide a \emph{compositional} and \emph{cost-aware} semantics which is based on factors, the standard mathematical tool used in Bayesian inference. Our results rely on advanced techniques rooted into linear logic, intersection types, rewriting theory, and Girard's geometry of interaction, which are here combined in a novel way.

==> 999_Commenti.tex <==
\newpage
\section{Commenti PER NOI }
In [Staton]  "The inference problem is to approximate the posterior distribution,
from the unnormalized posterior defined by the program, combining a prior and likelihood"

\subsection{Syntax}
\RED{\begin{proposition}\label{prop:uniqueness}
		Let $\tjudg{\Lambda}{\tm}{\iL}$. Then, there is a unique type derivation $\pi$ such that $\pi\dem\tjudg{\Lambda}{\tm}{\iL}$.
\end{proposition}}

\todocf{\RED{NB: the above statement is different from the statement in appendix}}




\todocf{Capire se mai lo usiamo davvero (penso di no)}


\CF{ The non-unicity of type derivations for ground terms, \textbf{even when context and type are given}, comes from the fact that observed names can be eliminated. However
	\begin{enumerate}
		\item eliminating observed variables  is against their use in  inference 
		\item In reality, we had non-unicity also before, if we had admitted terms $\true,\false$
		\item note that in both cases above, the simple types admit only one derivation
	\end{enumerate}
	
	\begin{itemize}
		\item Example of term which eliminates an observed variable:
		
		\[\letin{x}{\sample{p}}{\letin{z}{\obst{x}}{\CPT{z}}}:\Y  \]
		
		\item Examples of term that already in the current calculus ---if we did not exclude   boolean values from the terms we type--- would already admit several intersection type derivation:
		\begin{enumerate}
			\item $\letin  x {\sample p} {\sample q} $
			\item $\letin{x}{\sample{p}}{x}:T (\tor F \tor\X)$
			\item  $\letin{x}{\sample{p}}{\letin{z}{x}{\CPT{z}}}:\Y $
		\end{enumerate}
		We can type $x$  with  $\X$ or $T$ or $F$.
		
		\RED{ Note that the simple type derivation is unique!}
		
		
	\end{itemize}
}

\CF{
	\todocf{\RED{ \textbf{Claim }: All occurrence of name $\X$  in a type derivation $\pi$ have the same form, either are all $\X$, or all $\Xt$, or all $\Xf$.
		}
		
		\RED{\textbf{FALSE}!}
	}
	
	Esempi:
	\begin{enumerate}
		\item $  x_1:\Xt, x_2:\Xf \vdash \letin{z_1}{\obst{x_1}}{\letin{z_2}{\obsf{x_2}}{\pair{z_1}{z_2}}}: \Xt\otimes\Xf $
		
		\item Consideriamo il termine seguente (de-sugared in the obvious way). Le variabili $\Y_1,\Y_2$ dipendono entrambe da $\X$,
		ma i rispettivi fattori sono modificati in modo inconsistente
		\[  x_1:\Xt, x_2:\Xf \vdash \letin{z_1}{\obst{x_1}}{\letin{z_2}{\obsf{x_2}}
			{\pair {\CPTN{{\Y_1|\X}}{z_1}}{\CPTN{{\Y_2|X}}{z_2}}}}: \Y_1 \otimes\Y_2 \]
	\end{enumerate}
	
}

\paragraph{Il calcolo e' diverso da quelli di Delia \& Beniamino: usiamo massivamente side-effects}
\begin{enumerate}
	\item $ \letin{z}{\obst x}y $

	\item    $ \letin{x}{\coin{0.2}}{\letin{z}{\obst x}y}  $
\end{enumerate}

\subsection{Semantics of typed terms}


\CF{ ALTERNATIVA. \\
	Define: $\Supp \X=\{\true,\false\}, \Supp \Xt=\{\true\}, \Supp \Xf=\{\false\} $}
\blue{
	\begin{enumerate}
		\item $\icoin$ axiom 
		We associate to this axiom the  factor $\phi$ over the \pink{name}  $\set{\X}$ such that 
		$\phi (\x)\defeq\dist(\x)$  for each $\x\in \Supp{\XX}$, and $0$ otherwise.
		
		\item $\icond$ axiom. 
		We associate to this axiom the factor $\phi$ over the set of \pink{names} $\{\Y_1, \dots, \Y_n,\X\}$, such that 
		$\phi(\bvs\x)\defeq \dist_{\bvs}(\x)$,	 for each $\bvs\x\in \Supp{\YY_1} \times \dots\times  \Supp{\YY_n} \times \Supp{\XX}$, and $0$ otherwise.
\end{enumerate}}

\subsection{More Examples}
\begin{figure}
	\centering
	
	\[
	\begin{array}{|c|c|}
		\centering
		\arraycolsep=1.5pt
		%
		\coin{0.2}
		&
		\begin{array}{rl}
			\texttt{case} &{\rain}  \texttt{ of} \\
			&{\true} \caseSym \coin{0.7} \\
			&{\false}  \caseSym \coin{0.01}   
		\end{array}
		\\[4pt]
		\hline
		%
		\phi_1\defeq
		\begin{array}{|c|c|}
			\hline	
			\R  & \Pr (\R) \\
			\hline	
			\true	& 0.2 \\
			\false	& 0.8 \\
			\hline
		\end{array}
		\qquad	 &  \phi_2 \defeq 
		\begin{array}{|cc|c|}
			\hline	
			\R  & \W  & \Pr(\W | \R) \\
			\hline	
			\true  & \true	& 0.7 \\
			\true  & \false	& 0.3 \\
			\hline
			\false & \true	& 0.01 \\
			\false & \false	& 0.99 \\
			\hline
		\end{array}
		\\[4pt]
		\hline
		%
		\phi_1^\e= \phi_1
		&  \phi_2^\e =  
		\begin{array}{|cc|c|}
			\hline	
			\R  & \W  & \Pr(\W=\true | \R) \\
			\hline	
			\true  & \true	& 0.7 \\
			%	\true  & \false	& 0.3 \\
			\hline
			\false & \true	& 0.01 \\
			%	\false & \false	& 0.99 \\
			\hline
		\end{array}
		%
	\end{array}
	\]
	\caption{Dealing with evidence} %\label{fig:evidence}
\end{figure}

\subsection{Repository}

{\small 	\[\infer{\vdash \letin r {\coin {0.3}}  
		{\letin{w}{\CPT  r}{\pair r  w}}  :{ \R}\otimes { \W}}
	{ {\vdash \coin {0.2}:{\R}}   
		& 
		{ \infer{{r:{ \R} \vdash {\letin{w}{\CPT  r}{\pair r  w}}} :\R \otimes \W }
			{ r: \R \vdash \CPT  r: \RED{\W} & \infer{r:{ \R},   w: \W  \vdash \pair r  w : { \R}\otimes { \W}}
				{ r:{ \R} \vdash r:{ \R}  &   w:{ \W} \vdash  w:{ \W}} }    }}
	\]
}

{\small
	$\infer{\vdash \letp {\pair{r}{w}}  {u_1} {\letin {w'}{\obs {w}\true}{\pair r  {w'}}}} 
	{
		\infer{\vdash \letin r {\coin {0.2}}  
			{\letin{w}{\CPT  r}{\pair r  w}}  :{ \R}\otimes { \W}}
		{ {\vdash \coin {0.3}:{\R}}   
			& 
			{ \infer{{r:{ \R} \vdash {\letin{w}{\CPT  r}{\pair r  w}}} :\R \otimes \W }
				{ r: \R \vdash \CPT  r: \RED{\W} & \infer{r:{ \R},   w: \W  \vdash \pair r  w : { \R}\otimes { \W}}
					{ r:{ \R} \vdash r:{ \R}  &   w:{ \W} \vdash  w:{ \W}} }    }}
		&
		\infer{\vdash \letp {w'}{\obs {w}\true}{\pair r  {w'}}}
		{ w\vdash \obs {w}\true & r\vdash r}
	}
	$
}


==> 999_Repository.tex <==
\section{Repository}


\RED{\begin{proposition}\label{prop:uniqueness}
		Let $\tjudg{\Lambda}{\tm}{\iL}$. Then, there is a unique type derivation $\pi$ such that $\pi\dem\tjudg{\Lambda}{\tm}{\iL}$.
\end{proposition}}

\todocf{\RED{NB: the above statement is different from the statement in appendix}}




\todocf{Capire se mai lo usiamo davvero (penso di no)}


\CF{ The non-unicity of type derivations for ground terms, \textbf{even when context and type are given}, comes from the fact that observed names can be eliminated. However
	\begin{enumerate}
		\item eliminating observed variables  is against their use in  inference 
		\item In reality, we had non-unicity also before, if we had admitted terms $\true,\false$
		\item note that in both cases above, the simple types admit only one derivation
	\end{enumerate}
	
	\begin{itemize}
		\item Example of term which eliminates an observed variable:
		
		\[\letin{x}{\sample{p}}{\letin{z}{\obst{x}}{\CPT{z}}}:\Y  \]
		
		\item Examples of term that already in the current calculus ---if we did not exclude   boolean values from the terms we type--- would already admit several intersection type derivation:
		\begin{enumerate}
			\item $\letin  x {\sample p} {\sample q} $
			\item $\letin{x}{\sample{p}}{x}:T (\tor F \tor\X)$
			\item  $\letin{x}{\sample{p}}{\letin{z}{x}{\CPT{z}}}:\Y $
		\end{enumerate}
		We can type $x$  with  $\X$ or $T$ or $F$.
		
		\RED{ Note that the simple type derivation is unique!}
		
		
	\end{itemize}
}

\CF{
	\todocf{\RED{ \textbf{Claim }: All occurrence of name $\X$  in a type derivation $\pi$ have the same form, either are all $\X$, or all $\Xt$, or all $\Xf$.
		}
		
		\RED{\textbf{FALSE}!}
	}
	
	Esempi:
	\begin{enumerate}
		\item $  x_1:\Xt, x_2:\Xf \vdash \letin{z_1}{\obst{x_1}}{\letin{z_2}{\obsf{x_2}}{\pair{z_1}{z_2}}}: \Xt\otimes\Xf $
		
		\item Consideriamo il termine seguente (de-sugared in the obvious way). Le variabili $\Y_1,\Y_2$ dipendono entrambe da $\X$,
		ma i rispettivi fattori sono modificati in modo inconsistente
		\[  x_1:\Xt, x_2:\Xf \vdash \letin{z_1}{\obst{x_1}}{\letin{z_2}{\obsf{x_2}}
			{\pair {\CPTN{{\Y_1|\X}}{z_1}}{\CPTN{{\Y_2|X}}{z_2}}}}: \Y_1 \otimes\Y_2 \]
	\end{enumerate}
	
}



\cf{\subsection*{**  COMMENTS (for us)**}
	
	The condition on names is necessary both wrt  the relational model, and for the factor semantics to make sense.
	
	\begin{itemize}
		\item Consider of $x:\Bool, y:\Bool \vdash \pair x y : \Bool \otimes \Bool $
		\begin{itemize}
			\item 	Usual intersection types  admits 4 derivations:
			\begin{enumerate}
				\item $ \pi_1\dem_{\imin} x:\true, y:\true \vdash \pair x y : \true \otimes \true $
				
				\item $  \pi_2\dem_{\imin}  x:\true, y:\false \vdash \pair x y : \true \otimes \false $
				
				\item $ \pi_3\dem_{\imin}  x:\false, y:\false \vdash \pair x y : \false \otimes \false $
				\item $ \pi_4\dem_{\imin}  x:\false, y:\true \vdash \pair x y : \false \otimes \true $
			\end{enumerate}
			Said otherwise, the relational model  
			sends four of the $2^4$ tuples in $\Bool \times \Bool\larrow \Bool \times \Bool$ to 1, and four to 0.
			
			\item Consider the same as above in our Type system. 
			Point  (2.) in  names condition implies that a single derivation  provides all the four above
			\[x:\X, y:\Y \vdash \pair x y : \X \otimes \Y \]
			
			Without it, our  semantics of $x:\Bool, y:\Bool \vdash \pair x y : \Bool \otimes \Bool $ is wrong: it only sends two tuples to 1.
			
		\end{itemize}
		
		
		
\end{itemize}}


\subsection*{**MORE PRIVATE COMMENTS (for us)**}
\cf{
	\begin{fact}[to check]Assume  $\pi \dem_{\imin} \Lambda \vdash t:\iL$ and no main type has name $\Y$.
		\begin{enumerate}
			\item  If	$\Y \in \Nm{\Phi_\pi}$  than  $\Y\in \Lambda$.
			\item If $\Y\in \iL$ then $\Y\in \Lambda$
		\end{enumerate}
	\end{fact}
	
}
\begin{example}[Higher-Order term]
	
	\[\infer{\vdash \letin{f}{!u}{\Big( \letin{z}{\coin p}{(\der f)z} \Big)}:\Y  }
	{
		\infer[bang]{\pi_1 \dem \vdash \oc u: [\X \larrow \Y]}{\infer[abs]{\vdash u=\lam x.\CPT{x}   : \X \larrow \Y}{\infer[cond]{x:\X\vdash \CPT{x}:\Y}{}}}
		&
		\infer  {\pi_2\dem f: [\down \X \larrow  \up\Y]  \vdash ( \letin{z}{\coin p}{(\der f)z}): \down \Y}
		{\infer{\vdash \coin p: \X}{ }& \infer{z:\X, f:[\down \X \larrow  \up\Y] \vdash (\der f)z:\Y}
			{\infer{ f:[\X\larrow \Y] \vdash  \der f :\X\larrow \Y} {  f:[\X\larrow \Y] \vdash  f :[\X\larrow \Y ]} & z:\X\vdash z:\X}}
	}	
	\]
\end{example}

\begin{example}[Higher-Order]
	\[
	\pi_2'\dem	\infer {\vdash \lam f.\left( \letin{z}{\coin p}{(\der f)z}\right): [\down \X \larrow  \up\Y] \larrow \down \Y
	}{\pi_2\dem \infer {f: [\down \X \larrow  \up\Y]  \vdash \letin{z}{\coin p}{(\der f)z}: \down \Y}
		{\infer{\vdash \coin p: \X}{ }& \infer{z:\X, f:[\down \X \larrow  \up\Y] \vdash (\der f)z:\Y}
			{\infer{ f:[\X\larrow \Y] \vdash  \der f :\X\larrow \Y} {  f:[\X\larrow \Y] \vdash  f :[\X\larrow \Y ]} & z:\X\vdash z:\X}}}	
	\]
\end{example}			






==> biblio_to_check.tex <==
of SFPL [25]. It
bears some similarities with the adjoint calculus of [2], though we do not need
linear variables. It is also close to the Enriched Effect Calculus [10].

===============================

P. N. Benton and Philip Wadler. Linear logic, monads and the lambda calculus. In
Proceedings, 11th Annual IEEE Symposium on Logic in Computer Science, New
Brunswick, New Jersey, USA, July 27-30, 1996, pages 420{431. IEEE Computer
	Society, 1996.
	
	
	Jeff Egger, Rasmus Ejlers Møgelberg, and Alex Simpson. The enriched effect
	calculus: syntax and semantics. Journal of Logic and Computation, 24(3):615{654,
		2014.
		
		game  semantics    Recently, probabilisti programming
		
		
		@article{MelliesT10,
			author       = {Paul{-}Andr{\'{e}} Melli{\`{e}}s and
				Nicolas Tabareau},
			title        = {Resource modalities in tensor logic},
			journal      = {Ann. Pure Appl. Log.},
			volume       = {161},
			number       = {5},
			pages        = {632--653},
			year         = {2010},
			url          = {https://doi.org/10.1016/j.apal.2009.07.018},
			doi          = {10.1016/j.apal.2009.07.018},
			timestamp    = {Sun, 02 Oct 2022 15:27:35 +0200},
			biburl       = {https://dblp.org/rec/journals/apal/MelliesT10.bib},
			bibsource    = {dblp computer science bibliography, https://dblp.org}
		}
